A Parametric Study of the Coalescence of Liquid Drops in a Viscous Gas

The coalescence of two liquid drops surrounded by a viscous gas is considered in the framework of the conventional model. The problem is solved numerically with particular attention to resolving the very initial stage of the process which only recently has become accessible both experimentally and computationally. A systematic study of the parameter space of practical interest allows the influence of the governing parameters in the system to be identified and the role of viscous gas to be determined. In particular, it is shown that the viscosity of the gas suppresses the formation of toroidal bubble predicted in some cases by early computations where the gas' dynamics was neglected. Focussing computations on the very initial stages of coalescence and considering the large parameter space allows us to examine the accuracy and limits of applicability of various `scaling laws' proposed for different `regimes' and, in doing so, reveal certain inconsistencies in recent works. A comparison to experimental data shows that the conventional model is able to reproduce many qualitative features of the initial stages of coalescence, such as a collapse of calculations onto a `master curve' but, quantitatively, overpredicts the observed speed of coalescence and there are no free parameters to improve the fit. Finally, a phase diagram of parameter space, differing from previously published ones, is used to illustrate the key findings.

==> ArXiv Files/README <==
$Id: README 32701 2014-01-17 18:09:54Z karl $
This file is public domain.  (Originally written by Karl Berry, 2009.)

This is the README for the epstopdf script distribution.

Primary distribution point: http://mirror.ctan.org/support/epstopdf/
  (list of mirrors at: http://ctan.org/mirrors)

Home page: http://tug.org/epstopdf/

Run epstopdf --help for the usual list of options, examples, etc.

Mailing list for bugs and discussion: http://lists.tug.org/tex-k
When reporting bugs, please include an input file and command line
options, so the problem can be reproduced.

-------------------------------------------------------------------------
The test-binary and test-bin2 files were supplied by Akira Kakuto and
Reinhard Kotucha.  They contain binary data.  They are public domain.

The test-binhdr* files were supplied by Martin von Gagern, constructed
as follows.  They contain binary junk before the EPS starts.  We also
use these to test different line endings.  These files are public domain.

{ echo -e '%Some\000binary\001comment'; dot -Tps <<< 'digraph{a->b}'; }
  > test-binhdr-lf.eps
tr $'\n' $'\r' <test-binhdr-lf.eps >test-binhdr-cr.ps
unix2dos <test-binhdr-lf.eps >test-binhdr-cr.ps


==> README <==
$Id: README 32701 2014-01-17 18:09:54Z karl $
This file is public domain.  (Originally written by Karl Berry, 2009.)

This is the README for the epstopdf script distribution.

Primary distribution point: http://mirror.ctan.org/support/epstopdf/
  (list of mirrors at: http://ctan.org/mirrors)

Home page: http://tug.org/epstopdf/

Run epstopdf --help for the usual list of options, examples, etc.

Mailing list for bugs and discussion: http://lists.tug.org/tex-k
When reporting bugs, please include an input file and command line
options, so the problem can be reproduced.

-------------------------------------------------------------------------
The test-binary and test-bin2 files were supplied by Akira Kakuto and
Reinhard Kotucha.  They contain binary data.  They are public domain.

The test-binhdr* files were supplied by Martin von Gagern, constructed
as follows.  They contain binary junk before the EPS starts.  We also
use these to test different line endings.  These files are public domain.

{ echo -e '%Some\000binary\001comment'; dot -Tps <<< 'digraph{a->b}'; }
  > test-binhdr-lf.eps
tr $'\n' $'\r' <test-binhdr-lf.eps >test-binhdr-cr.ps
unix2dos <test-binhdr-lf.eps >test-binhdr-cr.ps

